Collapsibility and homological properties of $\mathfrak{I}$-contractible transformations

The family of $\mathfrak{I}$-contractible graphs and contractible transformations was defined by A. Ivashchenko in the mid-90's. In this paper we study the collapsibility and homological properties of the clique complex associated to $\mathfrak{I}$-contractible graphs. We show that for any graph in a special subfamily of the $\mathfrak{I}$-contractible graphs (the strong $\mathfrak{I}$-contractible ones) its clique complex is collapsible. Moreover, we present an algorithm that allows us to verify if any graph is strong $\mathfrak{I}$-contractible, as well as an algorithm to delete those vertices whose open neighborhood is also strong $\mathfrak{I}$-contractible. Finally, we show how to use these algorithms to compute the persistent homology of an arbitrary Vietoris-Rips complex for applications in topological data analysis.

==> 05-Acknowledgements.tex <==
\section*{Acknowledgments}
The author J.-F. Espinoza acknowledges the financial support of PRODEP and of the Universidad de Sonora, through the research project ``M\'etodos de Topolog\'ia Combinatoria en el An\'alisis de Datos''. 

The authors acknowledges all the observations of the anonymous referee, which were really pertinent to improve the presentation of this work. Special thanks for the editor, for the support and assistant in the submitting and preparation of this paper.

